MASS: Overcoming Language Bias in Image-Text Matching

Pretrained visual-language models have made significant advancements in multimodal tasks, including image-text retrieval. However, a major challenge in image-text matching lies in language bias, where models predominantly rely on language priors and neglect to adequately consider the visual content. We thus present Multimodal ASsociation Score (MASS), a framework that reduces the reliance on language priors for better visual accuracy in image-text matching problems. It can be seamlessly incorporated into existing visual-language models without necessitating additional training. Our experiments have shown that MASS effectively lessens language bias without losing an understanding of linguistic compositionality. Overall, MASS offers a promising solution for enhancing image-text matching performance in visual-language models.

==> 2-background.tex <==

\section{}


==> 2-relatedwork-short.tex <==
\section{Related Work}

\bfsection{Visual-Language Model}
Early visual-language models like LXMERT~\cite{tan2019lxmert} established visual-language alignment based on pretrained text encoder representations.
Later, the success of CLIP~\cite{Radford2021LearningTV} introduced contrastive learning as a core method for visual-language models, leading to further research like ALBEF~\cite{li2021align}, which incorporates contrastive loss as a part of its multi-task losses.
BLIP-2~\cite{li2023blip} demonstrated that frozen large language models can enhance image captioning performance. OFA~\cite{wang2022ofa} further extend visual-language models to a wider range of tasks including image generation. Recent visual instruction tuning models allow prompt-based control of visually conditioned knowledge.
LLaVA~\cite{liu2024visual} extend the pretrained language model LLAMA to multimodal inputs.
A prior study~\cite{lin2024revisiting} proposes a framework for mitigating language priors in vision-language models by introducing 'null images' and leveraging Pointwise Mutual Information (PMI), techniques similar to those presented in this work. Although both works share methodological elements, they were developed independently and address different objectives:~\cite{lin2024revisiting} focuses on theoretical contributions to vision-language alignment, while this work targets societal bias reduction and introduces new evaluation metrics, such as bias-aware Text-to-Image retrieval.

\bfsection{Bias in Multimodal Models}
Visual-language models often suffer from language bias induced by their training dataset. This deficiency has been explored as visual priming bias~\cite{zhang2016yin} and language prior~\cite{agrawal2018don}.
Language bias is also closely connected to socially offensive bias,
such as gender bias~\cite{de2021stereotype} and racial bias~\cite{davidson2019racial} in language models.
Social biases are also observed in the VLMs~\cite{hendricks2018women}.
Other works explore diverse categories~\cite{garcia2023uncurated} and metric extension~\cite{ross2021measuring} for social bias understanding.

\iffalse
\bfsection{Compositional Reasoning}
Various benchmarks have been suggested to test visual-language models' capability to handle visual-linguistic compositionality, including single noun difference understanding~\cite{shekhar2017foil}, comprehension of subject-verb-object relationships~\cite{hendricks2021probing}, sensitivity to the linguistic property perturbations~\cite{parcalabescu2022valse}. 
Aside from investigating linguistic properties, other works also explored
comparison of common attributes observed across multiple images~\cite{bogin2021covr} and identification of the difference between hard-negative images~\cite{thrush2022winoground}.
Recently, visual-language models such as CLIP have turned out to show weak language modeling capability~\cite{yuksekgonul2022and}.
In response, new benchmarks such as CREPE~\cite{ma2023crepe} and SugarCrepe~\cite{hsieh2024sugarcrepe} are proposed to measure the visual-linguistic compositionality of the models without incorporating linguistic bias.
\fi

==> 2-relatedwork_backup.tex <==
\section{Related Work}

\bfsection{Visual-Language Model}
Early visual-language models like ViLBERT~\cite{lu2019vilbert}, VisualBERT~\cite{li2019visualbert}, and LXMERT~\cite{tan2019lxmert} established visual-language alignment based on pretrained text encoder representations.
Later, the success of CLIP~\cite{Radford2021LearningTV} introduced contrastive learning as a core method for visual-language models, leading to further research like ALBEF~\cite{li2021align}, which incorporates contrastive loss as a part of its multi-task losses.
BLIP-2~\cite{li2023blip} demonstrated that aligning pretrained visual-language models with frozen large language models can enhance text generation. OFA~\cite{wang2022ofa} and UnifiedIO~\cite{lu2022unified} further extend visual-language models to a wider range of tasks including image generation.

Recently, visual instruction tuning models have been presented to allow prompt-based control of visually conditioned knowledge.
MiniGPT-4~\cite{zhu2023minigpt} and LLaVA~\cite{liu2024visual} extend the pretrained language model LLAMA~\cite{touvron2023llama} (and its variant Vicuna~\cite{chiang2023vicuna}) to multimodal inputs.
SVIT~\cite{zhao2023svit} scales up visual instruction tuning to more image-instruction pairs.
LLAMA-Adapter~\cite{zhang2023llama} and mPLUG-OWL~\cite{ye2023mplug} seek architectural and training-wise improvement of visual instruction tuning.
Otter~\cite{li2023mimic}, built on Flamingo architecture~\cite{alayrac2022flamingo, awadalla2023openflamingo}, can process multiple images and videos.
SEED~\cite{ge2023planting} and JAM~\cite{aiello2023jointly} enable text-to-image generation in the visual instructing tuning models.

\bfsection{Bias in Multimodal Models}
Visual-language models often suffer from language bias induced by their training dataset. This deficiency has been explored as visual priming bias~\cite{zhang2016yin, goyal2017making} and language prior~\cite{agrawal2018don, ramakrishnan2018overcoming}.
Language bias is also closely connected to socially offensive bias,
such as gender bias~\cite{de2021stereotype} and racial bias~\cite{davidson2019racial} in language models.
The social biases are observed in the VL models~\cite{hendricks2018women, wang2021gender, zhao2021understanding, birhane2021multimodal} as well.
Other works explore more diverse categories~\cite{garcia2023uncurated} and metric extension~\cite{ross2021measuring} for social bias understanding.

Social bias is an emerging problem in the text-to-image generation domain as well. DALL-Eval~\cite{cho2023dall} measures the gender and skin tone biases in recent text-to-image generation models to show that they reflect the biases in web image-text data. Seshadri~\etal~\cite{seshadri2023bias} shows that image generation models also amplify gender-occupation biases within the training data as image captioning models do.


\bfsection{Compositional Reasoning}
Various benchmarks have been suggested to test visual-language models' capability to handle visual-linguistic compositionality, including single noun difference understanding~\cite{shekhar2017foil}, comprehension of subject-verb-object relationships~\cite{hendricks2021probing}, sensitivity to the linguistic property perturbations~\cite{parcalabescu2022valse}. 
Aside from investigating linguistic properties, other works also explored
comparison of common attributes observed across multiple images~\cite{bogin2021covr} and identification of the difference between hard-negative images~\cite{thrush2022winoground}.
Recently, visual-language models such as CLIP have turned out to show weak language modeling capability~\cite{yuksekgonul2022and}.
In response, new benchmarks such as CREPE~\cite{ma2023crepe} and SugarCrepe~\cite{hsieh2024sugarcrepe} are proposed to measure the visual-linguistic compositionality of the models without incorporating linguistic bias.

==> 4-method_backup.tex <==
\section{Method}
\label{sec:method}

\subsection{Common Types of Confidence Score}

\noindent\textbf{Formulation}. Consider a visual-language model trained on the image-text pairs $(\mathbf{x}, \mathbf{y})$ in dataset $\mathcal{D}$. Here, $\mathbf{x}$ represents an image and $\mathbf{y}$ represents a text consists of variable-length token sequence $\{\mathbf{y}_i\}_{i \in \mathbb{N}}$, and each token $\mathbf{y}_i$ belong to vocabulary $\mathcal{V}$ with a size of $|\mathcal{V}|$. We consider two types of architecture of the visual-language model, the autoregressive architecture and the dual-encoder architecture.

The autoregressive visual-language model $f_{\theta}: \mathcal{V}| \mathcal{X} \times \mathcal{Y} \rightarrow \mathbb{R}^{|\mathcal{V}|}$ is trained by maximum likelihood estimation in general. More precisely, $f_{\theta}$ is trained to maximize the likelihood of the token sequence $\mathbf{y}$ by predicting likelihood of each token $\mathbf{y}_i$ on token distribution with given prefix $\mathbf{y}_{<i}$ and image $\mathbf{x}$ in autoregressive manner.

\begin{align}\label{eq1}
    f_{\theta} (\mathbf{y}|\mathbf{x}) = f_{\theta} ({\mathbf{y}_1} | \mathbf{x}) \prod_{i=2}^{|\mathbf{y}|} f_{\theta} 
    (\mathbf{y}_i|\mathbf{x}, \mathbf{y}_{<i})
\end{align}

The dual-encoder visual-language model which consists of two encoders, $g_{\phi}: \mathcal{X} \rightarrow \mathbb{R}^d$ and $h_{\gamma}: \mathcal{Y} \rightarrow \mathbb{R}^d$, is trained to maximize mutual information between image $\mathbf{x}$ and text $\mathbf{y}$, typically by InfoNCE loss. In this case, the exponential of the inner product between each encoder's output representation are designed to act as critic function which is proportional to ratio between joint distribution $p(\mathbf{x}, \mathbf{y})$ and product of each marginal distribution $p(\mathbf{x})p(\mathbf{y})$.

\begin{align}\label{eq2}
    \exp ( g_{\phi}(\mathbf{x})^{T} \cdot h_{\gamma}(\mathbf{y}) ) \propto \cfrac{p(\mathbf{x}, \mathbf{y})}{p(\mathbf{x})p(\mathbf{y})}
\end{align}

The problem of estimating the confidence of the model arises when observing a new image-text pair $(\mathbf{\bar{x}}, \mathbf{\bar{y}})$, as we want to determine how probable the model considers the observed pair to be \textit{correct} compared to those observed in the dataset $\mathcal{D}$. Formally, we want to estimate the probability of being \textit{correct} pair, with given $\mathbf{\bar{x}}$, $\mathbf{\bar{y}}$, $\mathbf{\theta}$. However, estimation of this probability is challenging, so various approaches attempt to estimate it by using a proximal confidence score estimator $\mathcal{C}(\cdot)$, which can be considered dependent on the desired quantity.

\begin{align}\label{eq3}
    \mathbb{P}(\textit{correct}|\mathbf{\bar{x}}, \mathbf{\bar{y}}, \theta) \rightarrow \mathcal{C}(\mathbf{\bar{x}}, \mathbf{\bar{y}}, \theta)
\end{align}

\noindent\textbf{Image-Text Classification Score}. One approach to estimate confidence score which we denote as Image-Text Classification (ITC) score is usually used on the encoder-decoder architecture. There are two variants for this score, based on the existence of classification head $l_{\theta}(\cdot)$ as subset of the model, which is trained to classify the \textit{correct} pairs in training process. If the model does not have such classification head, we can regard classification task as visual question answering task by comparing the likelihood $f_{\theta}(\cdot|\mathbf{\bar{x}}, \mathbf{\bar{y}})$ between \textit{yes} and \textit{no} token. 

\begin{align} %\label{eq4}
    \mathcal{C}_{\text{ITC}}(\mathbf{\bar{x}}, \mathbf{\bar{y}}, \theta)  & \coloneqq
    \begin{cases}
        l_{\theta}(\mathbf{\bar{x}}, \mathbf{\bar{y}})\\ \cfrac{f_{\theta}(\mathbf{y}_{\textit{yes}}|\mathbf{\bar{x}}, \mathbf{\bar{y}})}{\sum_{i \in \{\textit{yes}, \textit{no}\}} f_{\theta}(\mathbf{y}_{i}|\mathbf{\bar{x}}, \mathbf{\bar{y}})}
    \end{cases}
\end{align}

\noindent\textbf{Image-Text Similarity Score}. Another approach we denote as Image-Text Similarity (ITS) score is usually used on the dual-encoder architecture. After trained with contrastive loss, each output vector from image encoder and text encoder are regarded as cross-modal joint embedding. In this embedding space, similarity measure of two embedding can represent semantic similarity of the observation pair $\mathbf{\bar{x}}$ and $\mathbf{\bar{y}}$. Across the previous researches, the most popular choice for the similarity measure is cosine similarity, so we chose this as one type of confidence score estimator.

\begin{equation}\label{eq5}
    \mathcal{C}_{\text{ITS}}(\bar{\mathbf{x}}, \bar{\mathbf{y}}, (\phi, \gamma)) \coloneqq \cfrac{ g_{\phi}(\mathbf{x})^{T} \cdot h_{\gamma}(\mathbf{y}) }{|| g_{\phi}(\mathbf{x}) || \cdot ||h_{\gamma}(\mathbf{y})|| }
\end{equation}

\noindent\textbf{Token Likelihood Aggregation Score}. A straightforward way to understand the likelihood $f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}})$ is the probability of observed token sequence $\mathbf{\bar{y}}$ with given model parameter $\theta$, assuming the paired image $\bar{\mathbf{x}}$ has sampled in uniformly. In this sense, we can regard the likelihood $f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}})$ as confidence score estimator of the model. However, previous researches found that using likelihood from each token $\bar{\mathbf{y}}_i$ separately then aggregate them with pre-defined aggregation function $\text{agg}(\cdot)$ yields more fine-grained level confidence score estimator. We denote this approach as Token Likelihood Aggregation (TLA) score. In this case, we use the likelihood from token observation $\bar{\mathbf{y}}_i$ for given $\bar{\mathbf{x}}$ previous token sequence $\bar{\mathbf{y}}_{<i}$ and image $\bar{\mathbf{x}}$ with respect to the model parameter $\theta$. In previous approaches, the aggregation function $\text{agg}(\cdot)$ mainly chosen from $\text{sum}(\cdot)$, $\text{avg}(\cdot)$, $\text{max}(\cdot)$ and $\text{min}(\cdot)$. If we use $\text{prod}(\cdot)$ as the aggregation function, then this is equivalent to regard sequence level likelihood as the confidence score.

\begin{align}\label{eq6}
    \mathcal{C}_{\text{TLA}}(\bar{\mathbf{x}}, \bar{\mathbf{y}}, \theta) \coloneqq \text{agg}(f_{\theta}(\bar{\mathbf{y}}_i|\bar{\mathbf{y}}_{<i}, \bar{\mathbf{x}}))
\end{align}

\subsection{Pointwise Mutual Information Score}

\hspace*{2mm} The main problem of directly using likelihood as confidence score estimators is that it may not be suitable to measure the \textit{pure} contribution to the confidence of the model from given image $\bar{\mathbf{x}}$. Even if the likelihood of observation $\bar{\mathbf{y}}$ with respect to model parameter $\theta$ is not quite different whether $\bar{\mathbf{x}}$ is given or not, this estimator assign confidence score to the observation. This implies that naïve use of likelihood as confidence score does not exclude \textit{language bias} of the model. 

Formally, consider the likelihood of the model with given observation pairs, $f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}})$. From Bayes rules, we can decompose the likelihood to two distinctive terms, $f_{\theta}(\bar{\mathbf{y}})$ and $\frac{f_{\theta} (\mathbf{\bar{x}|\bar{y}}) }{f_{\theta} (\mathbf{\bar{x}})}$.

\begin{align}\label{eq7}
    f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}}) = f_{\theta}(\bar{\mathbf{y}}) \frac{f_{\theta}(\bar{\mathbf{x}}|\bar{\mathbf{y}})}{f_{\theta}(\bar{\mathbf{x}})}
\end{align}

We can consider the $f_{\theta}(\bar{\mathbf{y}})$ as the contribution from \textit{linguistic likelihood} of given observation $\mathbf{\bar{y}}$ to the likelihood of the pair. This is \underline{independent} property about the relation between image $\mathbf{\bar{x}}$ and text $\mathbf{\bar{y}}$, which can amplify the confidence score even the \textit{correspondence likelihood} $\frac{f_{\theta} (\mathbf{\bar{x}|\bar{y}}) }{f_{\theta} (\mathbf{\bar{x}})}$ was not influential. If the purpose was measuring the effect of given image $\mathbf{\bar{x}}$ to the confidence of model to observed $\mathbf{\bar{y}}$, this term should be regularized.

Therefore, the simple remedy for likelihood based approach would be dividing conditional likelihood $f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}})$ by the marginal likelihood $f_{\theta}(\bar{\mathbf{y}})$. If we consider this in log scale, this is equivalent to log-ratio between conditional likelihood $ f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}})$ from marginal likelihood $f_{\theta}(\bar{\mathbf{y}})$. If $f_{\theta}(\cdot|\cdot)$ is accurately estimating the ground-truth conditional image-text distribution of $p(\cdot|\cdot)$, this score is equivalent to estimating the pointwise mutual information, $\text{pmi}(\mathbf{x}; \mathbf{y})$. In this sense, we denote this new confidence score estimator as \textbf{Pointwise Mutual Information (PMI)} score. 

\begin{align}\label{eq8}
    \text{pmi}(\mathbf{x}; \mathbf{y}) \coloneqq \log \cfrac{p(\mathbf{x}, \mathbf{y})}{p(\mathbf{x}) p(\mathbf{y})} = \log \cfrac{p(\mathbf{y}|\mathbf{x})}{p(\mathbf{y})}
\end{align}

\begin{align}\label{eq9}
    \mathcal{C}_{\text{PMI}}(\bar{\mathbf{x}}, \bar{\mathbf{y}}, \theta) \coloneqq \log \cfrac{f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}})}{f_{\theta}(\bar{\mathbf{y}})}
\end{align}

Note that the target quantity with exponential function is proportional to the critic function of dual-encoder trained with contrastive learning used in ITS score. The dual-encoder architecture does not guarantee the critic function to be normalized, due to the energy-based modeling for Noise Constrastive Estimation (NCE) framework. This property made direct comparison of the scale of the critic function hard at the test time, so surrogate similarity measure such as cosine similarity should be used for score estimator. 

However, the autoregressive architecture decomposed the density $p(\mathbf{y}|\mathbf{x})$ to the tractable chain of token probability $p(\mathbf{y}_i|\mathbf{x}, \mathbf{y}_{<i})$, we can directly compare the pointwise estimation of target quantity as the score of the confidence if we can successfully estimate the marginal probability $p(\mathbf{y})$ by $f_{\theta}(\mathbf{y})$.

\subsection{Estimating the Marginal Probability}

\hspace*{2mm} The autoregressive visual language model $f_{\theta}$ assumes image input $\mathbf{x}$, we can only directly access to the likelihood $f_{\theta}(\mathbf{y}|\mathbf{x})$. Thus, one solution we can select is Monte Carlo approximation by uniformly sampling $N$ random image $\mathbf{\tilde{x}}$, then take the mean of each likelihood on text $\mathbf{y}$ with given $\mathbf{\tilde{x}}$ as approximation of the $f_{\theta}(\mathbf{y})$.

\begin{align}\label{eq10}
    f_{\theta}(\mathbf{y}) = \int_{\mathcal{X}} f_{\theta}(\mathbf{y}|\mathbf{x}) d\mathbf{x} \approx \cfrac{1}{N}\sum_{i=1}^N f_{\theta}(\mathbf{y}|\mathbf{\tilde{x}}_i)
\end{align}

However, this approach requires additional $N$ times of forward process to compute the score for one pair of the observation, also hard to guarantees the accuracy of the approximation compared to the computation cost. As the alternatives, we found that using image input as \textit{null image} $\mathbf{x}_{\emptyset}$, completely 'black-filled' image is good alternative to estimate $f_{\theta}(\mathbf{y})$ by $f_{\theta}(\mathbf{y}|\mathbf{x}_{\emptyset})$. For the rest of experiment, we used $f_{\theta}(\mathbf{y}|\mathbf{x}_{\emptyset})$ as the approximation of $f_{\theta}(\mathbf{y})$ to calculate the PMI score. 

\begin{align}\label{eq11}
    \mathcal{C}_{\text{PMI}}(\bar{\mathbf{x}}, \bar{\mathbf{y}}, \theta) \approx \log \cfrac{f_{\theta}(\bar{\mathbf{y}}|\bar{\mathbf{x}})}{f_{\theta}(\bar{\mathbf{y}}|\mathbf{x}_{\emptyset})}
\end{align}

==> 6-1-exp-debiasing_short.tex <==
\section{Experiments: Language Debiasing}
\label{sec:exp_bias}

We show that \modelname effectively reduces language bias in three different domains;
natural color association (\cref{subsec:exp_color}), object number counting (\cref{subsec:exp_number}), and gender balance in image search (\cref{subsec:exp_gender}).
The improvement is especially substantial when
the tested data have a different language bias from the training data
of the base visual-language model.

\bfsection{Backbones}
We use OFA~\cite{wang2022ofa} as the backbone VL model for both ITM, TL, and \modelname similarity functions.
Also, we experiment with alternative backbones of BLIP-2~\cite{li2023blip} and LLaVA~\cite{liu2024visual}. Note that ITM is not applicable for LLaVA since it only has the language modeling head.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.48\textwidth]{figure/fig_NCD_color_bias.pdf}
%     \caption{Description about how image-text pair is given to model. We compute difference between the score of 'fruit image-true caption' and 'fruit image-adversarial caption'}
%     \label{fig:fruit_gray}
% \end{figure}

    
%\begin{figure}[t]
%    \includegraphics[width=0.48\textwidth]{figure/fig_color.pdf}
%    \caption{Colour bias experiments on the Natural Colors Dataset~\cite{anwar2020image}. X-axis represents score differences which should be greater than zero.}%  x :  unmatching pair score - matching pair score, y: fruit type of NCD. large difference means less-biased for fruit color.}
%    \label{fig:exp_color}
%\end{figure}



% We find that our method's success on Imagescore (and groupscore because Imagescore is a bottleneck for groupscore on most of VL model and most of scoring method) is attributed to debiasing ability of our scoring scheme in language aspect. Table 6 shows VL model can concentrate more on objects in image, \\
% 
% 
% To estimate the capability of debiasing language prior inevitably gained through training process, we conducted 2 experiments that can prove language bias can be reduced by our method. We validate the hypotheses by two different experiment, colour debiasing and social(especially gender) debiasing.\\[10pt]


\input{figure/texfig_color}
\input{table/table_number2}

\subsection{Debiasing Colors}
\label{subsec:exp_color}

When there is linguistic bias in the data, the visual-language models trained on them would likely reflect the bias~\cite{birhane2021multimodal,ross2021measuring}.
However, evaluating the model for bias is not a simple problem:
how do we know when the model only relies on the text context without looking at the image?

Here, we devise a toy experiment where the model should perform perfectly if it truly looks at the image.
The Natural Color Dataset (NCD)~\cite{anwar2020image} is a dataset of various fruits colored either in the natural color or in gray.
Given a gray image of a fruit, we asked the model if the color is gray.
Surprisingly, the token likelihood score said no for many fruits and vegetables.


% It is likely that VL models have strong prior in color, [is BERT blind?] because most of images they learned would depict natural images(e.g Red apple), that would exist in real word, not learning unnatural images(e.g purple apple). To check whether our method can really reduce bias in color, we adopt NCD(Natural Color Dataset), which provides images of 20 types of fruits and vegetables paired with colors(also provide gray-colored version). \\
% Using same VL model(OFA) and differing only scoring method(TLC and ours), We feed 2 types of image-caption pair as input for model : ("The color of this {fruit} is gray", original image) and ("The color of this {fruit} is gray", gray-colored image),  then subtract the score of the former input from the score of the latter : score(caption, gray image) - score(caption, original image). Higher the difference, Less bias the model has, because high difference means that model can discriminate the color of fruit, more focusing on given visual information(fruit's gray color), not on language prior (fruit's original color). Figure 1 shows that using our method, comparing with TLC, VL model can concentrate more on visual information in all fruit type from NCD. \\[20pt]





\bfsection{Approach and metrics}
We use only the grayscale images from the NCD dataset, which leaves 723 images consisting of 20 different fruits.
Given an image, we build a true caption "The \textit{fruit} is gray." and an adversarial caption 
"The \textit{fruit} is \textit{color}.", in which \textit{fruit} and \textit{color} are variables replaced with the type of the fruit and its natural color.
%Given the grayscale image of a fruit or vegetable, we build the true caption "The \textit{fruit} is gray." and an adversarial caption "The \textit{fruit} is \textit{color}.".
Then, we compute the difference between the score of the true caption and that of the adversarial caption given the image.
Intuitively, the score should always be greater than zero for an image-text matching algorithm without severe language bias.

\bfsection{Results}
Fig~\ref{fig:color_bias} compares \modelname and token likelihood of the captioning model (TL) on the color debiasing experiment.
We report the ratio of the biased samples and the biased types (fruit or vegetable types of mean value lower than zero) here.
TL prefers its language bias over the image context in a third of the categories.
% On the other hand, TPMI, which alleviates the effect of language bias by suppressing the marginal likelihood, shows mean differences greater than zero for all categories.
In contrast, \modelname effectively reduces language bias, resulting in mean differences that are consistently above zero for all but one category.
% Note that while \modelname clearly reduces language bias, it cannot perfectly distinguish all biased samples.



\subsection{Debiasing Numbers}
\label{subsec:exp_number}


% \input{table/table_color}
\input{table/table_gender}

VL models are known to prefer specific numbers such as 0, 1, and 2~\cite{parcalabescu2021seeing},
regardless of the actual number of objects in an image.
Here, we test \modelname on the task of counting the number of visual entities.

%Thus, We additionally conduct an counting experiment to verify VL model can counts entities in image exactly beyond the training distribution, not distracted by prior incurred by imbalanced distribution in number. 

\bfsection{Approach}
We adopt the counting benchmark in VALSE dataset~\cite{parcalabescu2022valse}.
VALSE formulates counting tasks as foils. Given an image, a model is asked to differentiate the true caption with the correct number from the false caption with the wrong number (foil).
The benchmark consists of three sets: a set with balanced number distribution in the foils (\textit{balanced}), a set that only uses small numbers (\textit{small}), and a set in which true captions have only large numbers and foils have only small numbers (\textit{adversarial}). Note that models typically understand small numbers better since most images in training data do not have many objects. Hence, the \textit{adversarial} set is especially hard for models with language bias.
%in ~\cite{Parcalabescu2021VALSEAT}, which consists of various tasks that cover basic linguistic phenomena, we select tasks involving counting. They used Visual7W VQA dataset, and source its ‘how many’ examples whose answers are numerals. We followed experiment settings of ~\cite{Parcalabescu2021VALSEAT}.

\bfsection{Metric and baselines}
We report pairwise ranking accuracy metric, which formulates the counting task as an image-text alignment scoring problem.
Other baselines here include the multitask models such as LXMERT~\cite{tan2019lxmert} and 12-in-1~\cite{Lu_2020_CVPR}.

\bfsection{Results}
Table~\ref{tab:count} shows that our \modelname outperforms all baselines except one in all subsets.
Importantly, the score excels at the \textit{adversarial} set and performs on par with the best model 12-in-1.
As the \textit{adversarial} set is designed to be hard for models with language bias,
this result further verifies that the improvement of \modelname comes from language debiasing.

\subsection{Debiasing Genders}
\label{subsec:exp_gender}

We now turn to a more practical problem of balancing gender bias in image-text matching.
Here, we adopt the conventional experiment setup~\cite{wang2021gender} to evaluate the gender bias of a text-based image search algorithm.
The hypothesis is simple:
given a gender-neutral text query, the retrieved images should contain a similar number of men and women in them. % for the search algorithm to be unbiased.

\bfsection{Approach}
We evaluate our method in both text-to-image and image-to-text retrieval tasks using the test split of MS COCO dataset~\cite{chen2015microsoft}.\footnote{We use the Karpathy split~\cite{karpathy2015deep} with 5000 test images.}
Our text-to-image experiment follows Wang~\etal's setup. First, we \textit{neutralize} each caption in the dataset by replacing any gender-specific word with the corresponding gender-neutral alternatives. Then, we perform text-to-image retrieval on the COCO dataset using neutralized captions.

For the image-to-text retrieval task, we follow a similar approach; however, neither captions nor images are neutralized to align with the definition of the bias score described below. Instead, retrieval is performed using original captions. Neutralization of images (e.g., masking gender-related features) was avoided as it led to a loss of critical contextual information necessary for valid retrieval comparisons.
We utilize CLIP~\cite{Radford2021LearningTV} to retrieve the top 20 candidates, followed by re-ranking the list using image-text matching algorithms. This two-stage retrieval strategy is commonly adopted to improve evaluation efficiency~\cite{wang2022git,li2023blip}.

For the gender debiasing experiments, we include additional baselines from prior debiasing methods: SCAN~\cite{lee2018stacked}, FairSample~\cite{lee2018stacked}, and CLIP-clip~\cite{wang2021gender}. It should be noted that our results for the CLIP model differ from those reported by Wang~\etal due to the use of a larger model scale (ViT-Large in our study versus ViT-Base in theirs).

\bfsection{Metrics}
The \textit{bias score} suggested in Wang~\etal~compares the proportions of masculine and feminine images or captions in the search results.
When $N_{m}$ and $N_{f}$ are respectively the number of retrieved images or captions depicting male and female in dataset $D$, the bias score for the top $K$ retrieved results ($Bias@K$) is defined as follows:

\begin{align}
    f(x) &:= \begin{cases}
        0 & \text{if~} N_{m} + N_{f} = 0 \\
      \frac{N_{m} - N_{f}}{N_{m} + N_{f}} & \text{otherwise}
    \end{cases} \\
    &Bias@K := \frac{1}{|D|} \sum_{x \in D} f(x)
\end{align}

Note that the query $x$ is an image to retrieve a list of captions in image-to-text retrieval, and vice versa for text-to-image.
We use the words in captions to decide whether an image or caption contains gender-specific information: refer to Wang~\etal~\cite{wang2021gender} for more details.

We also evaluate the standard \textit{recall} metric as an indicator of correctness: for each query, recall is one when the retrieved samples contain any of the ground-truth image-text pairs and zero in the other case.
A good algorithm should be able to minimize bias and keep the recall high.

\bfsection{Results}
Table~\ref{tab:gender} summarizes the results of our gender debiasing experiments.
In the text-to-image setting, \modelname outperforms all other baselines by a wide margin in recall, while maintaining the bias score close to the best non-debiasing method (TL) of the baselines.
Also, while a previous debiasing-specific method (CLIP-clip) effectively ameliorates gender biases, it comes at an expanse of high degradation of recall accuracy.

On image-to-text retrieval, the captions retrieved by \modelname contained much more balanced gender keywords than the baselines.
Further, \modelname still shows the best recall among others, proving that its social bias reduction does not come at an expanse of correctness.
In conclusion, \modelname is the best option here for gender-debiased retrieval.

==> 7-results.tex <==
\section{Results}
\subsection{Main Results}
\subsection{Ablations}
\subsection{Analysis}

==> 8-limitation-short.tex <==
\section*{Broader Impact}
\label{sec:limitations}

The social bias reduction effect of \modelname has two important limitations.
First, it relies on the output of visual-language models, which may encode hidden biases.
Since \modelname is an inference-time method, it cannot audit the information stored in the models' parameters.
Hence, we acknowledge that while our framework can reduce social bias, the range and intensity of its effect
may vary with respect to the base VL model used.
Second, we only explore social bias in terms of language bias.
Social bias could be manifested as visual bias
or even in the form of bias that is identified only as combinations of image and text~\cite{yamada2022lemons}.
We hope this research serves as a simple but effective baseline 
to initiate a search for more robust approaches to social bias reduction 
in image-to-text alignment problems.

==> macro.tex <==
\newcommand{\todoc}[2]{{\textcolor{#1}{#2}}}
\newcommand{\todoblue}[1]{\todoc{blue}{#1}}

\newcommand{\todocc}[2]{{\textcolor{#1}{[[#2]]}}}
\newcommand{\todored}[1]{\todocc{red}{[[#1]]}}
\newcommand{\hist}[1]{\todored{hist: #1}}

\newcommand{\person}{{$\mathbb{P}$}}
\newcommand{\thought}{$\mathbb{Z}_{\mathbb{P}}$}
\newcommand{\se}{{\it SE}}%
\newcommand{\eg}{{\it e.g.,}}%
\newcommand{\ie}{{\it i.e.,}}%
\newcommand{\etal}{{\it et al.}}%
\newcommand{\etc}{{\it etc}}%
\newcommand{\ours}{\textbf{ReMemBot }}%
\newcommand{\memory}{\mathcal{M}}%
\newcommand{\carecall}{$\text{CareCall}_{mem}$}
\newcommand{\acpm}{$\mathbbm{A}^2$-CPM}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\definecolor{yellow-green}{rgb}{0.3, 0.5, 0.0}

% \newcommand{\concat}{\DOTSB\concat@\slimits@}

% Caligraphy style
\newcommand{\mcal}[1]{{\cal{#1}}}
\newcommand{\calA}{\mbox{${\cal A}$}}
\newcommand{\calB}{\mbox{${\cal B}$}}
\newcommand{\calC}{\mbox{${\cal C}$}}
\newcommand{\calD}{\mbox{${\cal D}$}}
\newcommand{\calE}{\mbox{${\cal E}$}}
\newcommand{\calF}{\mbox{${\cal F}$}}
\newcommand{\calG}{\mbox{${\cal G}$}}
\newcommand{\calH}{\mbox{${\cal H}$}}
\newcommand{\calI}{\mbox{${\cal I}$}}
\newcommand{\calJ}{\mbox{${\cal J}$}}
\newcommand{\calK}{\mbox{${\cal K}$}}
\newcommand{\calL}{\mbox{${\cal L}$}}
\newcommand{\calM}{\mbox{${\cal M}$}}
\newcommand{\calN}{\mbox{${\cal N}$}}
\newcommand{\calO}{\mbox{${\cal O}$}}
\newcommand{\calP}{\mbox{${\cal P}$}}
\newcommand{\calQ}{\mbox{${\cal Q}$}}
\newcommand{\calR}{\mbox{${\cal R}$}}
\newcommand{\calS}{\mbox{${\cal S}$}}
\newcommand{\calT}{\mbox{${\cal T}$}}
\newcommand{\calU}{\mbox{${\cal U}$}}
\newcommand{\calV}{\mbox{${\cal V}$}}
\newcommand{\calW}{\mbox{${\cal W}$}}
\newcommand{\calX}{\mbox{${\cal X}$}}
\newcommand{\calY}{\mbox{${\cal Y}$}}
\newcommand{\calZ}{\mbox{${\cal Z}$}}

\definecolor{lightblue}{RGB}{224,236,247}
\definecolor{deepblue}{RGB}{9,46,107}



==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> table/ax_table_svo-probe.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
         & \multicolumn{3}{c}{Text} & \multicolumn{3}{c}{Image} & \multicolumn{3}{c}{Group} \\
         Models
        & ITM/C & TL & \textbf{MASS}
        & ITM/C & TL & \textbf{MASS}
        & ITM/C & TL & \textbf{MASS}
        \\
        \hline
        Chance & \multicolumn{3}{c}{25.0} & \multicolumn{3}{c}{25.0} & \multicolumn{3}{c}{16.7} \\
        \hline
        CLIP & 61.1 & - & - & 38.3 & - & - & 31.8 & - & - \\
        \hline
        OFA\textsubscript{large}
        & 59.0 & 31.8 & 66.0
        & 47.5 & 21.5 & 50.1
        & 39.7 & 12.5 & 43.0\\
        \hline
        BLIP-2\textsubscript{T5}
        & 77.0 & 25.5 & 53.5
        & 52.1 & 32.0 & 71.2
        & 48.8 & 14.3 & 48.0 \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{OPT}
        & 77.0 & 23.3 & 54.4
        & 52.1 & 35.0 & 71.5
        & 48.8 & 14.3 & 48.6 \\
        \hline
        
        BLIP-2\textsubscript{coco}
        & 79.5 & - & -
        & 54.5 & - & -
        & 51.5 & - & - \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{pt-vitL}
        & 77.0 & - & -
        & 52.1 & - & -
        & 48.8 & - & - \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{pt-vitG}
        & 78.7 & - & -
        & 50.3 & - & -
        & 47.6 & - & - \\
        
    \end{tabular}

      \caption{Result on SVO-Probes dataset~\cite{hendricks2021probing}.
    %We composed 31,357 samples from 12,936 images (SVO-probe originally has 14,102 images, but some images are no longer accessible (the corresponding urls are corrupted).
    The best numbers are \textbf{bolded} and the second best ones are \underline{underlined}.}
    \label{tab:svo-probe}
\end{table}

==> table/ax_table_svo_temp.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ll|ccc}
        \multicolumn{2}{c}{Models} & Text & Image & Group \\
        \hline
        % \multicolumn{2}{l|}{Human} & 89.5 & 88.5 & 85.5 \\
        \multicolumn{2}{l|}{Chance} & 25.0 & 25.0 & 16.7 \\
        \hline
         
        CLIP & ITC & \underline{61.1} & 38.3 & 31.8 \\
        % LXMERT & ITM & - & - & - \\
        %CLIP\textsubscript{base} & ITC & 58.1 & 37.8 & 30.7 \\
        %CLIP\textsubscript{large} & ITC & 61.8 & 39.5 & 33.2 \\
        X-VLM & - & 72.7 & 56.6 & 51.7 \\
        albef & - &64.8 & 49.1 & 42.6 \\
        blip & - &71.8 & 51.4 & 46.5 \\
        
         \hline 
         \multirowcell{3}{OFA\textsubscript{large}}
         & ITM & 59.0 & \underline{47.5} & \underline{39.7}\\
         & TL & 31.8 & 21.5 & 12.5 \\
         & \modelname & \textbf{66.0} & \textbf{50.1} & \textbf{43.0} \\
         % OFA\textsubscript{large} & TPMI _{0.5} & 52.7 & 49.7 & 36.0 \\
         % & WTPMI & 32.3 & 23.3 & 13.8 \\
         %\hline
         %& $\Delta$ & +4.9 & +2.6 & +3.3 \\
         \hline 
 
         % OFA\textsubscript{large} & WTPMI_f & 49.1 & 37.6 & 29.4 \\
        
    \end{tabular}
    \caption{Result on SVO-probes dataset~\cite{hendricks2021probing}.
    %We composed 31,357 samples from 12,936 images (SVO-probe originally has 14,102 images, but some images are no longer accessible (the corresponding urls are corrupted).
    The best numbers are \textbf{bolded} and the second best ones are \underline{underlined}.}
    \label{tab:svo-probe-temp}
\end{table}

==> table/ax_table_winoground_blip.tex <==
\begin{table}
    \centering
    \begin{tabular}{ll|ccc}
        \multicolumn{2}{c}{Models} & Text & Image & Group \\
        \hline
        \multicolumn{2}{l|}{MTurk Human} & 89.5 & 88.5 & 85.5 \\
        \multicolumn{2}{l|}{Random Chance} & 25.0 & 25.0 & 16.7 \\
        \hline

        \multirowcell{4}{
          BLIP-2\\\textsubscript{FlanT5-xl}
          } & ITM & \textbf{42.8} & 19.0 & \underline{15.3} \\
         & TL & 22.3 & \underline{20.8} & 10.8 \\
         % & WTPMI  & 22.5 &  24.8 & 12.8 \\
         %& Ours-F & 28.7 & 30.0 & \textbf{19.2} \\
         & \modelname & \underline{26.3} & \textbf{33.3} & \textbf{18.0} \\
         & $\Delta$ & -16.5 & +14.3 & +2.7 \\
         \hline

          \multirowcell{4}{
          BLIP-2\\\textsubscript{OPT-2.7B}
          } & ITM & \textbf{42.8} & 19.0 & \underline{15.3} \\
         & TL & \underline{26.3} & \underline{23.5} & 12.9 \\
        %& WTPMI  & 24.5 & 28.5 & 14.8 \\
         %& Ours-F & 28.7 & 30.0 & \textbf{19.2} \\
         & \modelname & \underline{26.3} & \textbf{33.3} & \textbf{17.8} \\
         & $\Delta$ & -16.5 & +14.3 & +2.5 \\
         \hline
    \end{tabular}
    \caption{Winoground evaluation using BLIP-2 as the base VL model. The best numbers are \textbf{bolded} and the second best ones are \underline{underlined}. $\Delta$ denotes the difference between \modelname and ITM.}
    \label{tab:winoground_blip2}
\end{table}

==> table/backup_ax_table_winoground_tag_full.tex <==
\begin{table*}[ht]
\setlength{\tabcolsep}{2pt}
    \centering
    \tiny
    % \multicolumn{3}{c|}{\parbox{1.8cm}{\centering Ambiguously Correct}}
    \begin{tabular}{ll|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc}

& & \multicolumn{3}{c|}{\parbox{1.6cm}{\centering Non Compositional}} & \multicolumn{3}{c|}{\parbox{1.6cm}{\centering Ambiguously Correct}} & \multicolumn{3}{c|}{\parbox{1.6cm}{\centering Visually Difficult}} & \multicolumn{3}{c|}{\parbox{1.6cm}{\centering Unusual Text}} & \multicolumn{3}{c|}{\parbox{1.6cm}{\centering Complex Reasoning}} & \multicolumn{3}{c|}{\parbox{1.6cm}{\centering Unusual Image}} & \multicolumn{3}{c|}{\parbox{1.6cm}{\centering NoTag}} & \multicolumn{3}{c}{\parbox{1.6cm}{\centering Full}}\\
\multicolumn{2}{c|}{Models} & T & I & G & T & I & G & T & I & G & T & I & G & T & I & G & T & I & G & T & I & G & T & I & G\\
\hline
CLIP & ITM & 76.6 & 36.7 & 33.3 & 30.4 & 15.2 & 13.0 & 15.8 & 0.0 & 0.0 & 30.0 & 16.0 & 10.0 & 24.4 & 7.7 & 3.9 & 25.00 & 9.0 & 5.4 & 30.4 & 11.1 & 8.2 & 30.75 & 10.50 & 8.00\\

LXMERT & ITM & 10.0 &13.3& 3.3& 10.9 &2.2& 0.0& 21.1 & 7.9& 2.6& 10.0 & 6.0& 0.0& 16.7 & 3.9& 1.3& 12.5 & 7.1& 1.8& 19.9 & 4.7& 4.1 & 19.25 & 7.00 & 4.00\\ 

\hline

 & ITM & 46.7 & 36.7 & 26.7 & 28.3 & 17.4 & 13.0 & 23.7 & 13.2 & 5.3 & 22.0 & 16.0 & 10.0 & 16.7 & 9.0 & 1.3 & 16.1 & 7.1 & 7.1 & 30.8 & 19.2 & 10.5 & 26.3 & 16.5 & 9.5\\
 
OFA\textsubscript{large} & TL & 36.7 & 46.7 & 23.3 & 37.0 & 21.7 & \textbf{15.2} & 18.4 & 21.1 & 18.4 & 22.0 & 34.0 & 14.0 & 16.7 & 24.4 & \textbf{9.0} & 30.4 & 35.7 & \textbf{21.4} & 27.9 & 29.7 & 15.7 & 26.8 & 29.8 & 15.8\\
 
 & \modelname & 43.3 & 46.7 & \textbf{33.3} & 23.9 & 26.1 & 13.0 & 36.8 & 26.3 & \textbf{21.1} & 30.0 & 26.0 & \textbf{18.0} & 19.2 & 15.4 & 6.4 & 25.0 & 26.8 & 17.9 & 38.4 & 39.5 & \textbf{26.7} & 32.0 & 31.5 & \textbf{20.3}\\
 \hline

& ITM & 333.3& 16.7& 10.0&21.7& 8.7& 4.4&15.8& 15.8& 10.5&24.0& 22.0& 12.0&19.2& 3.9& 3.9&17.9& 9.0& 3.6&27.3& 12.8& 8.7&24.8& 11.8& 7.5\\
OFA\textsubscript{base} & TL & 46.7& 43.3& 26.7&15.2& 19.6& 6.5&26.3& 18.4& 15.8&18.0& 22.0& 12.0&14.1& 14.1& 5.1&35.7& 25.0& 16.1&27.3& 31.4& 15.1&23.8& 25.3& 12.5\\
 & \modelname & 50.0& 30.0& 26.7&32.6& 23.9& 21.7&26.3& 21.1& 13.2&18.0& 14.0& 4.0&16.7& 11.5& 5.1&28.6& 19.6& 14.3&36.6& 25.0& 18.6&30.3& 21.3& 15.3\\


 \hline
    \end{tabular}
    \caption{Results on Winoground~\cite{thrush2022winoground} benchmark categorized by reasons of difficulty~\cite{diwan2022winoground}. T, I, G denote \textit{Text}, \textit{Image}, and \textit{Groupscore}, respectively. The best numbers are \textbf{bolded} in \textit{Groupscore}.}  % result of LXMERT follows ~\cite{diwan2022winoground}}
    \label{tab:ax_winoground_tag}

\setlength{\tabcolsep}{6pt}

\end{table*}

%%% DATA
% OFA-L TPMI
% only_pmi {'ok': ([0.3953488372093023, 0.37209302325581395, 0.26744186046511625], 172), 'all': ([0.315, 0.32, 0.205], 400), 'Ambiguously Correct': ([0.2608695652173913, 0.2826086956521739, 0.13043478260869565], 46), 'Visually Difficult': ([0.2631578947368421, 0.3684210526315789, 0.21052631578947367], 38), 'Unusual Text': ([0.26, 0.3, 0.18], 50), 'Complex Reasoning': ([0.15384615384615385, 0.19230769230769232, 0.0641025641025641], 78), 'Unusual Image': ([0.26785714285714285, 0.25, 0.19642857142857142], 56), 'Non Minimal': ([0.4666666666666667, 0.36666666666666664, 0.3333333333333333], 30)}

% OFA-B TPMI
% only_pmi {'ok': ([0.2616279069767442, 0.37790697674418605, 0.20348837209302326], 172), 'all': ([0.21, 0.3175, 0.15], 400), 'Ambiguously Correct': ([0.15217391304347827, 0.30434782608695654, 0.08695652173913043], 46), 'Visually Difficult': ([0.13157894736842105, 0.2631578947368421, 0.07894736842105263], 38), 'Unusual Text': ([0.14, 0.28, 0.08], 50), 'Complex Reasoning': ([0.0641025641025641, 0.20512820512820512, 0.05128205128205128], 78), 'Unusual Image': ([0.25, 0.30357142857142855, 0.14285714285714285], 56), 'Non Minimal': ([0.3333333333333333, 0.4666666666666667, 0.23333333333333334], 30)}

==> table/table_color.tex <==
\begin{table}
    \centering
    \begin{tabular}{ll|>{\centering\arraybackslash}m{1.8cm}
    >{\centering\arraybackslash}m{1,8cm}}
        \multicolumn{2}{c}{Models} & \% samples biased $\downarrow$ & \% types biased $\downarrow$ \\
        % \hline
        % CLIP & ITC & 0.00 & 0.00 \\
        \hline
        \multirowcell{2}{OFA\textsubscript{large}}
         % & ITM & 1.25 & 0.00 \\
         & TL & 16.78 & 33.33 \\
         & \modelname & 2.36 & 0.00 \\
         \hline 
 
         % OFA\textsubscript{large} & WTPMI_f & 49.1 & 37.6 & 29.4 \\
        
    \end{tabular}
    \caption{Color debiasing experiment in Natural Colors Dataset~\cite{anwar2020image}. \modelname debiases TL.}
    \label{tab:color}
\end{table}

==> table/table_comp.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
         & \multicolumn{3}{c}{Text} & \multicolumn{3}{c}{Image} & \multicolumn{3}{c}{Group} \\
         Models
        & ITM/C & TL & \textbf{MASS}
        & ITM/C & TL & \textbf{MASS}
        & ITM/C & TL & \textbf{MASS}
        \\
        \hline
        Human & \multicolumn{3}{c}{89.5}  & \multicolumn{3}{c}{88.5}  & \multicolumn{3}{c}{85.5} \\
        Chance & \multicolumn{3}{c}{25.0} & \multicolumn{3}{c}{25.0} & \multicolumn{3}{c}{16.7} \\
        \hline
        VinVL & 37.8 & - & - & 17.8 & - & - & 14.5 & - & - \\
        LXMERT & 19.3 & - & - & 7.0 & - & - & 4.0 & - & - \\
        CLIP & 30.8 & - & - & 10.5 & - & - & 8.0 & - & - \\
        \hline
        OFA\textsubscript{large}
        & 26.4 & 26.8 & \textbf{32.0}($\uparrow$5.2)
        & 16.5 & 29.8 & \textbf{31.5}($\uparrow$2.7)
        & 9.5 & 15.8 & \textbf{20.3}($\uparrow$4.5)\\
        \xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{base}
        & 26.8 & 23.8 & \textbf{30.3}($\uparrow$3.5)
        & 10.8 & \textbf{25.3} & 21.3($\downarrow$4.0)
        & 6.5 & 12.5 & \textbf{15.3}($\uparrow$2.8) \\
        \xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{tiny}
        & \textbf{22.8} & 15.5 & 18.0 ($\downarrow$4.8)
        & 7.8 & 14.8 & \textbf{17.5} ($\uparrow$2.7)
        & 4.5 & 5.0 & \textbf{8.0} ($\uparrow$3.0)\\
        \hline
        BLIP-2\textsubscript{T5}
        & \textbf{42.5} & 22.8 & 26.8($\downarrow$15.7)
        & 19.5 & 21.5 & \textbf{32.0}($\uparrow$10.5)
        & 15.5 & 11.0 & \textbf{18.0}($\uparrow$2.5) \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{OPT}
        & \textbf{42.5} & 23.3 & 22.8($\downarrow$19.7)
        & 19.5 & 24.8 & \textbf{29.8}($\uparrow$5.1)
        & \textbf{15.5} & 12.5 & 15.0($\downarrow$0.5) \\
        \hline

        BLIP-2\textsubscript{coco}
        & 44.0 & - & -
        & 25.8 & - & -
        & 23.5 & - & - \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{pt-vitL}
        & 42.5 & - & -
        & 19.5 & - & -
        & 15.5 & - & - \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{pt-vitG}
        & 43.0 & - & -
        & 21.8 & - & -
        & 18.0 & - & - \\
        \hline
    \end{tabular}
    \caption{Results on Winoground~\cite{thrush2022winoground}.
    The best matching algorithm for each model is marked \textbf{bold}. } % $\Delta$ denotes the improvement of \modelname over ITM.}
    \label{tab:comp}
\end{table}

==> table/table_multimodal-predicate-noun-dependencies.tex <==
\begin{table}
    \centering
    \begin{tabular}{ll|cccc}
        \multicolumn{2}{c}{Models} & Acc(Text)  & Image  & Group  \\
        \hline
        \multicolumn{2}{l|}{Chance} & 25.0  & 25.0 & 16.7 \\
        \hline
        LXMERT & & 57 & 58.7 & 44.6  \\
        UNITER &  & 54 & - & -\\
        ViLBERT &  & 28 & - & -\\
        ViLT &  & 40 & - & -\\
        Oscar &  & 32 & - & -\\
        VinVL &  & 30 & - & -\\
        CLIP &  & 20 & 53.4 & 20.2 \\
        
        \hline

         %& TLC-A & 47.7  \\
         %OFA\textsubscript{large} & Ours-M & 40.9  \\
         %& Ours-F & \textbf{53.4}  \\
         
         \multirowcell{3}{OFA\textsubscript{large}}
         & ITM & \textbf{72.0} & 73.1 & \textbf{60.1} \\
         & TL & 44.8 & 48.5 & 31.9 \\
        % & WTPMI & 39.9  \\
         & TPMI & 54.3 & 53.9 & 40.5 \\
         \hline
                 


    \end{tabular}
    \caption{MPND original paper ~~, in here, ~~}
    \label{tab:np}
\end{table}


% OFA-large-caption
% {'tl': 0.46826625386996906,
% 'tpmi': 0.48993808049535603,
% 'wtpmi': 0.3993808049535604,
% 'wtpmi_f': 0.49613003095975233,
% 'clip': 0.19659442724458204}

==> table/table_number.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
         & \multicolumn{3}{c}{Hard} & \multicolumn{3}{c}{Small} & \multicolumn{3}{c}{Adv.} \\
         Models
        & ITM/C & TL & \textbf{MASS}
        & ITM/C & TL & \textbf{MASS}
        & ITM/C & TL & \textbf{MASS}
        \\
        \hline
        Chance & \multicolumn{3}{c}{16.7} & \multicolumn{3}{c}{16.7} & \multicolumn{3}{c}{16.7} \\
        \hline
        CLIP & 62.1 & - & - & 62.5 & - & - & 57.5 & - & - \\
        LXMERT & 62.2 & - & - & 69.2 & - & - & 42.6 & - & - \\
        12-in-1 & 76.7 & - & - & 80.2 & - & - & 77.3 & - & - \\
        \hline
        OFA\textsubscript{large}
        & 66.8 & 65.4 & 70.0($\uparrow$3.2)
        & 71.7 & 71.1 & 73.2($\uparrow$1.5)
        & 72.0 & 66.8 & 76.7($\uparrow$4.7)\\
        \hline
        BLIP-2\textsubscript{T5}
        & 68.0 & 59.3 & 63.6
        & 69.8 & 66.1 & 67.4
        & 77.6 & 58.6 & 72.0 \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{OPT}
        & 68.0 & 63.3 & 58.3
        & 69.8 & 65.6 & 63.3
        & 77.6 & 62.2 & 70.2 \\
        \hline
        BLIP-2\textsubscript{coco}
        & 71.7 & - & -
        & 78.6 & - & -
        & 77.0 & - & - \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{pt-vitL}
        & 68.0 & - & -
        & 69.8 & - & -
        & 77.6 & - & - \\
        \xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\xspace\textsubscript{pt-vitG}
        & 71.2 & - & -
        & 78.1 & - & -
        & 80.7 & - & - \\
        
    \end{tabular}
    \caption{Counting experiment in VALSE dataset~\cite{Parcalabescu2021VALSEAT}. Adv. denotes the adversarial set with explicit language bias. The best numbers are \textbf{bolded} and the second best ones are \underline{underlined}.}
    \label{tab:count}
\end{table}

==> table/table_svo-probe_subset.tex <==
\begin{table}
    \centering
    \begin{tabular}{ll|cccc}
        \multicolumn{2}{c}{Models} & Subject & Verb & Object & Total
        \\
        \hline
        \multicolumn{2}{l|}{Random Chance} & 16.7 & 16.7 & 16.7 \\
        \hline
        CLIP\textsubscript{base} & ITC & 38.0 & 26.2 & 38.8 & 30.7\\
        \hline

        \multirowcell{3}{OFA\textsubscript{large}}
         & ITM & 47.5 & 27.2& 59.0  & 37.0\\
         & TL & 19.1 & 5.5 & 15.1  & 9.6\\
        % & WTPMI & 20.3 & 16.2 & 18.0 \\
         & TPMI & 44.7 & 34.4 & 53.1  & 39.9\\
         \hline

    \end{tabular}
    \caption{Evaluation on 3 subset from SVO-probe. The subsets are comprised based on "which word is modified in original caption?". We only report Groupscore here.  Appendix shows overall result across 3 subsets.}
    \label{tab:svo-probe_subset}
\end{table}



==> table/table_winoground.tex <==
\begin{table}
    \centering
    \begin{tabular}{ll|ccc}
        \multicolumn{2}{c}{Models} & Text & Image & Group \\
        \hline
        \multicolumn{2}{l|}{Human} & 89.5 & 88.5 & 85.5 \\
        \multicolumn{2}{l|}{Chance} & 25.0 & 25.0 & 16.7 \\
        \hline
        VinVL & ITM & \textbf{37.8} & 17.8 & 14.5 \\
        LXMERT & ITM & 19.3 & 7.0 & 4.0 \\
        CLIP & ITC & 30.8 & 10.5 & 8.0 \\
        \hline
         \multirowcell{3}{OFA\textsubscript{large}} & ITM & 26.4 & 16.5 & 9.5 \\
         & TL & 26.8 & 29.8   & \underline{15.8} \\
        % OFA\textsubscript{large} & W\modelname & 25.2 & \textbf{33.0} & 18.0 \\
        %Large & W\modelname & 25.2 & \textbf{33.0} & 18.0 \\
         %& Ours-F & 28.7 & 30.0 & \textbf{19.2} \\
         & \modelname & \underline{32.0} & \textbf{31.5} & \textbf{20.3} \\
         % & \modelname\textsubscript{0.5} & \textbf{34.8} & \textbf{31.5} & \textbf{21.3} \\
         %& $\Delta$ & +5.6 & +15.0 & +10.8 \\
         \hline
                 
         \multirowcell{3}{OFA\textsubscript{base}}& ITM & 26.8 & 10.8 & 6.5 \\
         & TL & 23.8 & \underline{25.3} & 12.5 \\
        % Base & W\modelname & 23.0 & 28.7 & \textbf{15.0} \\
         %& Ours-F & 22.0 & \textbf{31.0} & \textbf{15.0} \\
         & \modelname & 30.3 & 21.3 & 15.3 \\
         % & \modelname\textsubscript{0.5} & 28.5 & \textbf{21.3} & 14.8 \\
         % & $\Delta$ & +3.5 & +10.5 & +8.3 \\
         \hline
         
         \multirowcell{3}{OFA\textsubscript{tiny}} 
         & ITM & 22.8 & 7.8 & 4.5 \\
         & TL & 15.5 & 14.8 & 5.0 \\
        % Tiny & W\modelname & 14.8 & 17.0 & 6.8 \\
         % & Ours-F & 18.0 & \textbf{20.0} & \textbf{10.0} \\
         & \modelname & 18.0 & 17.5 & 8.0 \\
         % & \modelname\textsubscript{0.5} & 19.5 & \textbf{17.5} & \textbf{9.3} \\
         % & $\Delta$ & -3.3 & +9.7 & +4.8 \\
         \hline
    \end{tabular}
    \caption{Results on Winoground~\cite{thrush2022winoground}.
    The best numbers are \textbf{bolded} and the second best ones are \underline{underlined}.
    } % $\Delta$ denotes the improvement of \modelname over ITM.}

    \label{tab:winoground}
\end{table}

==> table/table_winoground_vis_2.tex <==
\begin{table*}[t]
\centering
    \begin{tabular}{l|cccc}
    Image & 
    \multicolumn{2}{c}{\includegraphics[width=4.5cm]{figure/winoground_img/90_image0.png} }&
    \multicolumn{2}{c}{\includegraphics[width=4.5cm]{figure/winoground_img/90_image1.png}}\\

    \hline
     Method &  Caption & score &  Caption & score\\
    \hline


  
    \rule{0pt}{0.7cm}\multirow{2}{*}{PMILD} & 
    \multirow{4}{*}{\includegraphics[width=5cm]{figure/winoground_cap/90_0_.png} } & \textbf{1.45} &
    \multirow{4}{*}{\includegraphics[width=5cm]{figure/winoground_cap/90_1_.png} } & 1.13  \\
    \rule{0pt}{0.6cm}&& 0.35 && \textbf{1.38}\\
    \rule{0pt}{0.7cm}\multirow{2}{*}{TL}&& 0.05 && \textbf{0.13}\\
    \rule{0pt}{0.6cm}&& \textbf{0.45} && 0.11\\
  
    \hline
    \hline
    Image & 
    \multicolumn{2}{c}{\includegraphics[width=4.5cm]{figure/winoground_img/90_image0.png}}&
    \multicolumn{2}{c}{\includegraphics[width=4.5cm]{figure/winoground_img/90_image1.png}}\\

    \hline
     Method &  Caption & score &  Caption & score\\
    \hline


  
    \rule{0pt}{0.67cm}\multirow{2}{*}{PMILD} & 
    \multirow{4}{*}{\begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.0cm}}
    \includegraphics[width=5cm]{figure/winoground_cap/10_0.png}
    \end{adjustbox} } & \textbf{1.17} &

    
    \multirow{4}{*}{\includegraphics[width=5cm]{figure/winoground_cap/10_1.png} } & 0.98  \\
    \rule{0pt}{0.67cm}&& 0.86 && \textbf{1.39}\\
    \rule{0pt}{0.67cm}\multirow{2}{*}{TL}&& 0.19 && \textbf{0.138}\\
    \rule{0pt}{0.67cm}&& \textbf{0.12} && 0.131\\
    
    




    
    \hline
    \end{tabular}
\caption{an example of winoground dataset with OFA, comparing each scoring method(TLC and ours). Intensity of word's color means how much VL model give confidnece score to that word(token). Between two sentences, one that matches to image is underlines.}
\label{tab:winoground_visualize}
\end{table*}

% base
% 0.05
% 0.45
% 0.13
% 0.11
% 
% ours
% 1.45
% 0.35
% 1.13
% 1.38

==> table/table_winoground_visualize.tex <==
\begin{table*}[t]
\centering
    	
    \begin{tabular}{l|cccc}
    Image & 
    \multicolumn{2}{c}{\includegraphics[width=6cm]{figure/winoground_img/90_image0.png} }&
    \multicolumn{2}{c}{\includegraphics[width=6cm]{figure/winoground_img/90_image1.png}}\\

    \hline
     Method &  Caption & score &  Caption & score\\



  

  
    \hline
    \multirow{2}{*}{PMILD} & 
    \begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.2cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_0.PNG}\end{adjustbox} &1.0&
    \begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.2cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_4.PNG}\end{adjustbox}& 1.0\\
    
    &\begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.1cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_1.PNG}\end{adjustbox} &1.0&
    \begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.1cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_5.PNG}\end{adjustbox} &1.0\\
    
     
    \hline
    \multirow{2}{*}{TL} & 
    \begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.2cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_1.PNG}\end{adjustbox} &1.0&
    \begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.2cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_5.png}\end{adjustbox} &1.0\\
    
    &\begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.1cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_2.PNG}\end{adjustbox} &1.0&
    \begin{adjustbox}{margin={0cm, 0cm, 0cm, 0.1cm}}\includegraphics[width=5cm]{figure/winoground_cap/90_6.PNG}\end{adjustbox} &1.0\\
     
    \hline
    \end{tabular}
\caption{an example of winoground dataset with OFA, comparing each scoring method(TLC and ours). Intensity of word's color means how much VL model give confidnece score to that word(token). Between two sentences, one that matches to image is underlines.}
\label{tab:winoground_visualize}
\end{table*}
